Hyper-Representations: Learning from Populations of Neural Networks

This thesis addresses the challenge of understanding Neural Networks through the lens of their most fundamental component: the weights, which encapsulate the learned information and determine the model behavior. At the core of this thesis is a fundamental question: Can we learn general, task-agnostic representations from populations of Neural Network models? The key contribution of this thesis to answer that question are hyper-representations, a self-supervised method to learn representations of NN weights. Work in this thesis finds that trained NN models indeed occupy meaningful structures in the weight space, that can be learned and used. Through extensive experiments, this thesis demonstrates that hyper-representations uncover model properties, such as their performance, state of training, or hyperparameters. Moreover, the identification of regions with specific properties in hyper-representation space allows to sample and generate model weights with targeted properties. This thesis demonstrates applications for fine-tuning, and transfer learning to great success. Lastly, it presents methods that allow hyper-representations to generalize beyond model sizes, architectures, and tasks. The practical implications of that are profound, as it opens the door to foundation models of Neural Networks, which aggregate and instantiate their knowledge across models and architectures. Ultimately, this thesis contributes to the deeper understanding of Neural Networks by investigating structures in their weights which leads to more interpretable, efficient, and adaptable models. By laying the groundwork for representation learning of NN weights, this research demonstrates the potential to change the way Neural Networks are developed, analyzed, and used.

==> 0E_list_of_abbreviations.tex <==
\clearpage

\renewcommand{\rightmark}{List of Abbreviations}
\renewcommand{\leftmark}{List of Abbreviations}


\chapter*{List of Abbreviations} 
\thispagestyle{plain}
\vspace{-1.0cm}
\begin{footnotesize}
\begin{longtable}{>{\raggedright\arraybackslash} p{0.2\linewidth} p{0.6\linewidth} >{\centering\arraybackslash} p{0.1\linewidth}}
% \caption{Abbreviations}
\label{tab:basic_thesis_abbreviations} \\
\endfirsthead

\multicolumn{3}{c}%
{{}} \\
\endhead

\multicolumn{3}{r}{{Continued on next page}} \\
\endfoot

\endlastfoot
\textbf{AE} & Adversarial Autoencoder \\
\textbf{Adam} & Adaptive Moment Estimation \\
\textbf{AI} & Artificial Intelligence \\
\textbf{AN} & Artificial Neuron \\
\textbf{ANN} & Artificial Neural Network \\
\textbf{CE} &  Cross Entropy \\
\textbf{CL} & Contrastive learning \\
\textbf{CNN} & Convolutional Neural Network \\
\textbf{DL} & Deep Learning \\
\textbf{EMA} & Exponential Moving Average \\
\textbf{GAN} & Generative Adversarial Network \\
\textbf{GPU} & Graphic Processing Unit \\
\textbf{LLM} & Large Language Model \\
\textbf{ML} & Machine Learning \\
\textbf{MSE} & Mean Squared Error \\
\textbf{NT-Xent} & Normalized Temperature-Controlled Cross-Entropy \\
\textbf{PCA} & Principal Component Analysis \\
\textbf{SSL} & Self-Supervised Learning \\
\textbf{SVD} & Singular Value Decomposition \\
\textbf{VAE} & Variational Autoencoder \\
\textbf{VQ-VAE} & Vector Quantized-Variational Autoencoder \\

\end{longtable}
\end{footnotesize}

\addcontentsline{toc}{chapter}{Appendix A: List of Abbreviations}

\newpage

==> 0H_list_of_symbols.tex <==
\clearpage

\renewcommand{\rightmark}{List of Symbols}
\renewcommand{\leftmark}{List of Symbols}

\chapter*{List of Symbols} 
\thispagestyle{plain}
\vspace{-1.0cm}
\begin{footnotesize}
\begin{longtable}{>{\raggedright\arraybackslash} p{0.15\linewidth} p{0.6\linewidth} >{\centering\arraybackslash} p{0.1\linewidth}}
\caption{Symbols and descriptions.}
\label{tab:basic_thesis_symbols} \\
\toprule
\textbf{Symbol} & \textbf{Description} & \textbf{Chapter} \\
\midrule
\endfirsthead

\multicolumn{3}{c}%
{{\tablename\ \thetable{} -- continued from previous page} \vspace{0.5cm}} \\
\toprule
\textbf{Symbol} & \textbf{Description} & \textbf{Chapter} \\
\midrule
\endhead % This header will appear on every new page
    
\multicolumn{3}{r}{{Continued on next page}} \\
\endfoot

\endlastfoot

    %\textbf{Datasets and Their Variants:} \\
    $\mathcal{D}$ & Population of accounting journal entries & 3, 4, 5 \\
    $\hat{\mathcal{D}}$ & Population of pre-processed accounting journal entries & 3, 4, 5 \\
    $\tilde{\mathcal{D}}$ & Population of reconstructed accounting journal entries & 3, 4, 5 \\
    
    %\textbf{Entities and Their Attributes:} \\
    $x_{i}$ & Accounting journal entry & 3, 4, 5 \\
    $x_{i}^{j}$ & Attribute of accounting journal entry & 3, 4, 5 \\
    $x_{i}^{a}$ & Categorical attribute of accounting journal entry & 3, 4, 5 \\
    $x_{i}^{b}$ & Numerical attribute of accounting journal entry & 3, 4, 5 \\
    $\hat{x}_{i}$ & Preprocessed accounting journal entry & 3, 4, 5 \\
    $\hat{x}_{i}^{j}$ & Preprocessed attribute of accounting journal entry & 3, 4, 5 \\
    $\upsilon_{i}$ & One-hot encoded dimension of accounting journal entry & 3, 4, 5 \\
    $z_{i}$ & Latent representation of accounting journal entry & 3, 4, 5 \\
    $z_{i}^{j}$ & Latent representation dimension of accounting journal entry & 3, 4, 5 \\
    $\tilde{x}_{i}$ & Reconstructed accounting journal entry & 3, 4, 5 \\
    $\tilde{x}_{i}^{j}$ & Reconstructed attribute of accounting journal entry & 3, 4, 5 \\

    %\textbf{Neural Network Components and Their Parameters:} \\
    $f_{\theta}$ & Neural network model with parameters $\theta$ & 3, 4, 5 \\
    $q_{\psi}$ & Encoder neural network model with parameters $\psi$ & 3, 4, 5 \\
    $p_{\phi}$ & Decoder neural network model with parameters $\phi$ & 3, 4, 5 \\
    $\mathcal{Z}$ & Continuous latent space representation & 3, 4, 5 \\
    $\calL$ & Count of fully-connected neural network layers & 3, 4, 5 \\
    $\ell$ & Layer in a fully-connected neural network & 3, 4, 5 \\
    $W^{\ell}$ & Weights for layer $\ell$ in the neural network & 3, 4, 5 \\
    $b^{\ell}$ & Biases for layer $\ell$ in the neural network & 3, 4, 5 \\
    $\sigma$ & Activation function of the artificial neuron & 3, 4, 5 \\
    $\alpha_{relu}$ & Scaling factor for the Leaky ReLU activation function & 3, 4, 5 \\
   
    %\textbf{Model Optimization and Regularization Parameters:} \\
    $\mathcal{B}$ & Count of model optimization batches & 3, 4, 5 \\
    $\rho$ & Batch size used in model optimization & 3, 4, 5 \\
    $\eta$ & Learning rate used in model optimization & 3, 4, 5 \\
    $\zeta$ & Iterations used in model optimization & 3, 4, 5 \\
    $p_{drop}$ & Dropout probability used in model optimization & 3, 4, 5 \\
    $\beta_{1}, \beta_{2}$ & Exponential decay rates used in ADAM model optimization & 3, 4, 5 \\
    $\vartheta$ & Regularization factor of the reconstruction loss attribute & 3, 4, 5 \\
    $\beta_{AS}$ & Regularization factor of the anomaly score & 3, 4, 5 \\
    
    %\textbf{Anomaly-Related Metrics:} \\
    $\alpha_{1}$ & Count of global accounting anomalies. & 3, 4, 5 \\
    $\alpha_{2}$ & Count of local accounting anomalies. & 3, 4, 5 \\

\\

    $\gamma_{AS}$ & Threshold parameter for anomaly score & 3.1, 3.2 \\
\\
    $\eta_{ema}$ & Decay parameter for exponential moving average & 3.2 \\
    $\pi_{k}$ & Count of the nearest latent embeddings & 3.2 \\
    $c_{k}$ & Count of the exponential moving average embeddings & 3.2 \\
\\
    $z_{e}$ & Latent journal entry representation in continuous form & 3.2, 3.3 \\
    $z_{q}$ & Latent journal entry representation in discrete form & 3.2, 3.3 \\
    $e_{i}$ & Latent journal entry embedding in normalized form & 3.2, 3.3 \\
    $\bar{e}_{k}$ & Latent journal entry embedding in discrete form & 3.2, 3.3 \\
    $\mathcal{Z}_{e}$ & Latent space in discrete form & 3.2, 3.3 \\
    $\alpha_{vae}, \beta_{vae}, \gamma_{vae}$ & Regularization factors of the quantized reconstruction loss & 3.2, 3.3 \\
\\
    $x^{q}_{i}$ & Accounting journal entry query & 3.3 \\
    $z^{q}_{i}$ & Accounting journal entry representation query & 3.3 \\
    $e^{q}_{i}$ & Accounting journal entry embedding query & 3.3 \\
    $\mathcal{Z}_{h}$ & Latent space in normalized form & 3.3 \\
    $x^{+}, x^{-}$ & Positive and negative augmented journal entries & 3.3 \\
    $z^{+}, z^{-}$ & Positive and negative augmented representations & 3.3 \\
    $e^{+}, e^{-}$ & Positive and negative augmented embeddings & 3.3 \\
    $\tau^{+}, \tau^{-}$ & Positive and negative augmentations & 3.3 \\
    $\mathcal{P}^{+}, \mathcal{P}^{-}$ & Positive and negative augmentation policies & 3.3 \\
    $g_{\gamma}$ & Projection neural network model with parameters $\gamma$ & 3.3 \\
    $\tau_{nce}$ & Temperature parameter for noise contrastive estimation & 3.3 \\
    $\mu_{R}, \mu_{C}, \mu_{G}$ & Means for noise, cut, and gaussian augmentations & 3.3 \\
    $\sigma_{R}, \sigma_{G}$ & Standard deviations for noise and gaussian augmentations & 3.3  \\


\\

    $y_{i}$ & Class label of prior distribution & 4.1, 4.2 \\
    $\tilde{y}_{i}$ & Class label predicted from prior distribution & 4.1, 4.2 \\
    $p_{d}$ & Prior distribution of accounting journal entries & 4.1, 4.2 \\
    $p_{n}$ & Prior noise sampling distribution & 4.1, 4.2 \\
    $q_{z}$ & Posterior distribution of latent representations & 4.1, 4.2 \\
    $z_{\tau}$ & Gaussian distribution of the latent posterior & 4.1, 4.2 \\
    $d_{\omega}$ & Discriminator neural network with parameters $\omega$ & 4.1, 4.2 \\
    $\tau$ & Gaussian $\mathcal{N}_{\tau}$ in the prior noise sampling distribution & 4.1, 4.2 \\
    $\mu_{\tau}, \sigma_{\tau}$ & Mode and standard deviation of Gaussian $\mathcal{N}_{\tau}$ & 4.1, 4.2 \\

    $\check{\mathcal{D}}$ & Population of synthetic accounting journal entries & 4.2 \\
    $\mathcal{D}^{\text{Adv}}$ & Population of adversarial accounting journal entries & 4.2 \\
    $\check{x}_{i}$ & Synthetic accounting journal entry & 4.2 \\
    $x_{i}^{\text{Adv}}$ & Adversarial accounting journal entry & 4.2 \\
    $z_{i}^{\text{Adv}}$ & Latent space sample of adversarial accounting journal entry & 4.2 \\
    $\check{z}_{i}$ & Latent space sample of synthetic accounting journal entry & 4.2 \\
    $\delta$ & Step-size for Euclidean sampling & 4.2 \\
    $\lambda_{1}$ & Threshold for attribute sampling map & 4.2 \\
    $\lambda_{2}$ & Threshold for robust sampling map & 4.2 \\
\\    
    $h_{\omega}$ & Hiding neural network with parameters $\omega$ & 4.3\\
    $\alpha_{\text{SG}}, \beta_{\text{SG}}$ & Regularization factors for steganography loss & 4.3 \\
    $I^{pre}$ & Secret image of the steganography & 4.3 \\
    $I^{con}$ & Container image of the steganography & 4.3 \\
    $I^{cov}$ & Cover image of the steganography & 4.3 \\
    $I^{rev}$ & Revealed image of the steganography & 4.3 \\

\\

    $\mathcal{D}^{iid}$ & Population of iid distributed accounting journal entries & 5 \\
    $\mathcal{D}^{niid}$ & Population of non-iid distributed accounting journal entries & 5 \\
    $\mathcal{J}$ & Count of departments generating city payments & 5 \\
    $A_{j}$ & Department generating city payments & 5\\
\\
    $q', p'$ & Sub-networks of the private encoder and decoder network & 5.1\\
    $q*, p*$ & Sub-networks of the public encoder and decoder network & 5.1\\
    $\ell_{c}$ & Cut-layer of the neural networks & 5.1\\
    $\ell^{q}_{c}, \ell^{p}_{c}$ & Cut-layers of the encoder and decoder network & 5.1\\
    $\nabla_{max}$ & Maximum norm threshold of the per-sample gradients & 5.1\\
    $\mu_{dp}, \sigma_{dp}$ &  Mean and standard deviation of the differential privacy noise & 5.1\\
    $\kappa$ & Regularization factor of the differential privacy noise & 5.1\\
\\
    $\mathcal{D}_{i}$ & Population of the \textit{i}-th client's accounting journal entries &  5.1, 5.3 \\
    $\xi$ & Server in federated learning &  5.1, 5.3 \\
    $\omega_{i}$ & Client in federated learning & 5.1, 5.3 \\
    $f_{\theta}^{\xi}$ & Central neural network model with parameters $\theta^{\xi}$ & 5.1, 5.3 \\
    $f_{\theta, i}^{\omega}$ & Decentral neural network model with parameters $\theta_{i}^{\omega'}$ &  5.1, 5.3 \\
    $\mathcal{C}$ & Count of federated clients &  5.1, 5.3 \\
    $\lambda$ & Count of selected federated clients &  5.1, 5.3 \\
    $\mathcal{R}$ & Count of communication rounds in federated learning &  5.1, 5.3 \\
    $r$ & Communication round in federated learning &  5.1, 5.3 \\
    $\theta^{\omega *}$ & Public model parameters of the federated client & 5.1, 5.3 \\
    $\theta^{\omega '}$ & Private model parameters of the federated client &  5.1, 5.3 \\
    $\hbar$ & Sampling factor of random experience payment sampling & 5.2\\
\\    
    %\textbf{Others:} \\
    $\mathcal{D}^{(t)}$ & Population of $t$-th period's accounting journal entries & 5.2, 5.3 \\
    $T$ & Count of time periods in continual learning & 5.2, 5.3 \\
    $t$ & Time period in continual learning & 5.2, 5.3 \\
    $E^{(t)}$ & Experience in continual learning & 5.2, 5.3 \\
    $f^{(t)}_{\theta^{(t)}}$ & Experience neural network model with parameters $\theta^{(t)}$ & 5.2, 5.3 \\
    $\lambda_{EWC}$ & Regularization factor of the elastic weight consolidation & 5.2, 5.3 \\
    $[B]$ & Replay buffer of the experience replay & 5.2, 5.3 \\
    $N_{ER}$ & Replay buffer size of the experience replay & 5.2, 5.3 \\
\\
    $\lambda_{\scalebox{0.5}{LwF}}$ & Regularization factor of the learning without forgetting & 5.3 \\
    $\lambda_{\scalebox{0.5}{Prox}}$ & Regularization factor of the federated proximal learning & 5.3 \\
    $\lambda_{\scalebox{0.5}{Scaf}}$ & Regularization factor of the federated scaffold learning & 5.3 \\
    $\beta_{1}^{\scalebox{0.5}{Yogi}}$, $\beta_{2}^{\scalebox{0.5}{Yogi}}$ & Exponential decay rates of the federated yogi learning & 5.3 \\
    $\tau_{\scalebox{0.6}{Yogi}}$ & Temperature parameter of the federated yogi learning & 5.3 \\
% \vspace{0.2cm}
\bottomrule
\end{longtable}
\end{footnotesize}

\addcontentsline{toc}{chapter}{Appendix B: List of Symbols}

\newpage

==> 0_statutory_declaration.tex <==
\chapter*{Statutory Declaration} 

\normalsize `I hereby declare,

\begin{itemize}
    \item that I have written this thesis independently;
    \item that I have written the articles and contributions using only the aids listed in the index;
    \item that all parts of the thesis produced with the help of aids (including AI tools) have been precisely declared;
    \item that I have mentioned all sources used and cited them correctly according to established academic citation rules; this also includes the comprehensive disclosure of all personal publications;
    \item that I have acquired all immaterial rights to any materials I may have used, such as images or graphics, or that these materials were originally created by myself;
    \item that I am aware of the legal provisions regarding the publication and dissemination of parts or the entire thesis and that I comply with them accordingly;
    \item that I am aware that the University will prosecute a violation of this Declaration of Authorship and that disciplinary as well as criminal consequences may result, which may lead to expulsion from the University or to the withdrawal of my title.'
\end{itemize}

\noindent By submitting this thesis, I confirm through my conclusive action that I am submitting the statutory declaration, that I have read and understood it, and that it is true.

\vspace{1.0cm}

Place and data of issue: \hspace{4cm} Signature:

\vspace{0.5cm}

St. Gallen, 13.06.2024

\addcontentsline{toc}{chapter}{Statutory Declaration}

\newpage


==> chapters/chapter_1_weight_space/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> chapters/chapter_2_model_zoos/99_checklist.tex <==
\newpage
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, in Section \ref{sec:model_zoos:generation}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{The method we propose is a general machine learning method. It comes with all the risks involved, but in our opinion does not pose any particular risk.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{In the corresponding github.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes, in section \ref{app:zoo_generation} and in the published code.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report mean and standard deviation for all results.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Details on the dataset generation are reported in Appendix \ref{app:zoo_generation}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{I.e., the image datasets}
  \item Did you mention the license of the assets?
    \answerNo{The image datasets we use are common machine learning datasets,  which is why we refrain from mentioning their license.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The main contribution is the dataset, which we make available online.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{No personal data was used for this work.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{The datasets contain no personal information. As we use common machine learning datasets they also do not contain offensive content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{Our experiments do not rely on crowdsourcing nor did we conduct research on human subjects.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{Our experiments do not rely on crowdsourcing nor did we conduct research on human subjects}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{Our experiments do not rely on crowdsourcing nor did we conduct research on human subjects}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> chapters/chapter_4_generative_hyper_representations/checklist.tex <==
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:gen_hyper_reps:limitations} and ~\ref{sec:gen_hyper_reps:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{The method we propose is a general machine learning method. It comes with all the risks involved, but in our opinion does not pose any particular risk.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
     \answerYes{Code, hyper-representations of selected model zoos are included in the supplemental material}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All the details are specified in the Appendix \ref{app:zoos} and~\ref{app:training}.}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report means and std for all experiments in the main paper and provide additional details about median, CI95 on the median, p-value and effect size in the Appendix~\ref{app:results}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{app:training}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See Section ~\ref{app:zoos}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We have trained new model zoos and will make them publicly available via an URL}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{Our experiments use publicly available image datasets, which we cite. The model zoos and code for hyper-representation learning was published on github and zenodo by the authors of the original paper under Creative Commons Attribution 4.0.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Our experiments rely on common computer vision datasets and do not contain personally identifiable information nor offensive content.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> chapters/chapter_4_generative_hyper_representations/table_id.tex <==
\begin{table}[t]
\begin{minipage}[t]{0.98\textwidth}
\centering
{\small
\begin{tabular}{l|ccc|cc}
\toprule
\multicolumn{6}{c}{\textbf{Version 1 - ID only}}  \\
\multicolumn{6}{c}{\texttt{In-Distribution Experiments - Accuracies}}  \\
 & MNIST & SVHN & USPS & CIFAR-10 & STL-10 \\
\midrule
$B_T$ & 0.911 [0.911, 0.912] & 0.723 [0.720, 0.724] & 0.922 [0.921, 0.922] & 0.444 [0.444, 0.444] & 0.555 [0.555, 0.555]\\ 
%\midrule
$B_F$ & 0.912 [0.910, 0.913] & 0.732 [0.728, 0.734] & 0.922 [0.921, 0.923] & 0.444 [0.444, 0.444] & 0.555 [0.555, 0.555]\\ 
\midrule
$S_{N30}$ & \textbf{0.940 [0.939, 0.941]} & \textbf{0.765 [0.763, 0.767]} & 0.911 [0.911, 0.913] & 0.444 [0.444, 0.444] & 0.555 [0.555, 0.555]\\ 
%\midrule
$S_{D30}$ & 0.932 [0.931, 0.933] & 0.742 [0.739, 0.745] & \textbf{0.925 [0.924, 0.926]} & 0.444 [0.444, 0.444] & 0.555 [0.555, 0.555]\\ 
\end{tabular}
}
\caption{Accuracy of sampled models: median and 95\% confidence intervals. }
\label{tab:gen_hyper_reps:accuracy_static_id}
\end{minipage}
\vspace{-.2in}
\end{table}


\begin{table}[t]
\begin{minipage}[t]{0.98\textwidth}
\centering
{\small
\begin{tabular}{l|ccc|cc}
\toprule
\multicolumn{6}{c}{\textbf{Version 1 - ID only}}  \\
\multicolumn{6}{c}{\texttt{In-Distribution Experiments - Statistical Hypothesis Test}}  \\
 & MNIST & SVHN & USPS & CIFAR-10 & STL-10 \\
\midrule
$S_{D30}$ vs. $B_T$ & 8.6e-73 | 0.9689 & 1.6e-30 | 0.7985 & 7.0e-10 | 0.6601 & 0.444 | 0.444  & 0.555 | 0.555 \\ 
%\midrule
$S_{N30}$ vs. $B_T$ & 5.6e-82 | 0.9983 &  4.7e-76 | 0.9797 & 1.7e-42 | 0.1450 & 0.444 | 0.444  & 0.555 | 0.555 \\ 
\midrule
$S_{D30}$ vs. $B_F$ & 4.0e-45 | 0.9707 & 3.0e-08 | 0.6850 & 2.9e-04 | 0.6208 & 0.444 | 0.444  & 0.555 | 0.555 \\ 
%\midrule
$S_{N30}$ vs. $B_F$ & 1.5e-50 | 0.9983 & 1.7e-42 | 0.9563 & 3.6e-28 | 0.1326 & 0.444 | 0.444  & 0.555 | 0.555 \\ 
\end{tabular}
}
\caption{Mann-Whitney U test of Samples S vs Baselines B: p-value and CLES (Common Language Effect Strength). p-values indicate the probability of the samples of two groups originating from the same distribution. CLES=0.5 indicates no effect, CLES=1.0 a strong positive, CLES=0.0 a strong negative effect.
As the results indicate, both proposed sampling methods are almost always statistically significantly better than the two baselines. Further, their effect is often very strong. 
}
\label{tab:gen_hyper_reps:test_static_id}
\end{minipage}
\vspace{-.2in}
\end{table}

==> chapters/chapter_4_generative_hyper_representations/table_ood.tex <==
\begin{table}[t]
\begin{minipage}[t]{0.98\textwidth}
\centering
\caption{\small Mean and standard deviation of the accuracy (\%) of the populations trained on image classification tasks \textbf{after fine-tuning}. On the main diagonal are in-distribution experiments, otherwise out-of-distribution from source to target. 
%$B_T$ denotes the baseline trained directly on the target dataset. 
% The other populations have at least 50 members each. 
%$B_F$ is the second baseline pre-trained on source and fine-tuned on target. 
%$S_{\text{Distr}}$ is the distribution-based, %$S_{\text{Neigh}}$ the neighborhood-based, and %$S_{\text{GAN}}$ the GAN-based sampling method. 
% The suffix $30$ indicates that the sampling method was based on the top 30 \% of the train set. 
Bold numbers highlight the best source-to-target results. 
% Confidence intervals, p-values and effect size can be found in the Appendix.
% $B_T$ denotes the baseline with 700 members trained directly on the target dataset. The other populations have at least 50 members each. $B_F$ is the second baseline pre-trained on source and fine-tuned on target. $S_{\text{Distr}}$ is the distribution based sampling method, $S_{\text{Neigh}}$ the neighborhood based sampling method. The suffix $30$ indicates that the sampling method was based on the top 30 \% of the train set. Bold numbers highlight the best source-to-target results. Confidence intervals, p-values and effect size can be found in the Appendix.
}
\label{tab:gen_hyper_reps:accuracies}
{\scriptsize
\setlength{\tabcolsep}{8pt}
\begin{tabular}{lccccccc}
\toprule
% \multicolumn{5}{c}{\textbf{Version 2 - ID+OOD}}  \\
 &\multicolumn{4}{c}{\texttt{Digit Classification}} & \multicolumn{3}{c}{\texttt{Natural Image Classification}}  \\
 \cmidrule(r){2-5} \cmidrule(l){6-8}
% \midrule
Population & Source & \multicolumn{3}{c}{\texttt{Target}}  & Source & \multicolumn{2}{c}{\texttt{Target}} \\
\cmidrule(r){1-1} \cmidrule(rl){2-2} \cmidrule(rl){3-5} \cmidrule(rl){6-6}  \cmidrule(l){7-8}
% \midrule
            &                           & MNIST                     & SVHN                     & USPS                       &                            & CIFAR-10                     & STL-10 \\
% \midrule
\cmidrule(rl){3-5}  \cmidrule(l){7-8}
From scratch ($B_T$)      &                           & 91.1 | 0.95               & 70.7 | 8.80              & \textbf{92.2 | 0.58}       &                            & \textbf{48.7 | 1.38} 	    &         39.0 | 1.02 \\
% \midrule
\cmidrule(r){1-1} \cmidrule(rl){2-2}  \cmidrule(rl){3-5} \cmidrule(rl){6-6} \cmidrule(l){7-8}
% $B_T$     & MNIST                     & 0.911               & 0.222           & 0.333 \\ 
Fine-tune ($B_F$)       & \multirow{7}{*}{MNIST}    & 91.1 | 0.88               & 76.1 | 1.35              & 79.3 | 1.85                & \multirow{7}{*}{CIFAR-10} &  48.3 | 1.26                  & \textbf{42.7 | 1.22} \\  
% \hdashline
% \cmidrule(r){1-1}  \cmidrule(rl){3-5}  \cmidrule(l){7-8}
$S_{\text{Distr}}$     &                           & 92.5 | 0.75               & 76.4 | 1.55              & 79.2 | 2.17                &                            & 48.0 | 1.16                  &         40.6 | 1.07 \\
$S_{\text{Distr}30}$   &                           & 93.0 | 0.68               & \textbf{77.1 | 1.45}     & \textbf{80.8 | 0.83}       &                            & \textbf{48.6 | 0.53 }        &         41.1 | 0.93 \\
$S_{\text{Neigh}}$     &                           & 93.3 | 0.52               & 76.8 | 1.07              & 78.5 | 1.46                &                           &  45.2 | 1.33                  &         36.5 | 1.98 \\
$S_{\text{Neigh}30}$   &                           & \textbf{94.0 | 0.56}      & 76.7 | 1.32              & 79.6 | 1.31                &                           &   46.2 | 0.81                 &         37.9 | 1.57 \\ 
$S_{\text{GAN}}$     &                           & 93.5 | 0.60               & 74.6 | 11.32             & 78.9 | 1.64                &                           & 46.1 | 0.96                   &         38.6 | 1.41 \\
$S_{\text{GAN}30}$   &                           & 93.8 | 0.63               & 76.5 | 1.75              & 80.0 | 1.32                &                           & 46.7 | 0.87                   &         38.4 | 1.35 \\
% \midrule
\cmidrule(r){1-1} \cmidrule(rl){2-2}  \cmidrule(rl){3-5} \cmidrule(rl){6-6} \cmidrule(l){7-8}
Fine-tune ($B_F$)       & \multirow{7}{*}{SVHN}     & 95.0 | 0.78               & 72.4 | 6.36              & 87.1 | 1.68                & \multirow{7}{*}{STL-10}    & \textbf{49.2 | 0.70 	}       & \textbf{39.2 | 1.01}   \\  
% \hdashline
% \cmidrule(r){1-1}  \cmidrule(rl){3-5}  \cmidrule(l){7-8}
$S_{\text{Distr}}$     &                           & 95.0 | 0.81               & 71.8 | 7.68              & 87.0 | 1.72                &                             & 48.7 | 0.77                 & 37.4 | 1.28 	   \\ 
$S_{\text{Distr}30}$   &                           & \textbf{95.5 | 0.40}      & 74.2 | 1.39              & \textbf{88.3 | 1.09}       &                            & 48.8 | 0.90                   & 38.1 | 1.13   \\ 
$S_{\text{Neigh}}$     &                           & 95.9 | 9.85               & \textbf{77.9 | 1.40}      & 88.3 | 1.96                &                            & 10.0 | 0.00                  & 28.5 | 2.43  \\  
$S_{\text{Neigh}30}$   &                           & 95.5 | 0.68               & 76.4 | 1.02              & 85.8 | 1.49                &                            & 48.9 | 0.67 	                & 38.0 | 1.14 	   \\  
$S_{\text{GAN}}$     &                           & 94.3 | 0.87               & 74.3 | 1.39              & 82.3 | 2.63                &                             & 49.0 | 0.77 	                & 38.3 | 1.21 	   \\
$S_{\text{GAN}30}$   &                           & 94.9 | 0.72               & 75.1 | 1.24              & 84.3 | 2.22                &                             & xx.x | x.xx 	                & 38.2 | 0.96 	   \\  
% \midrule
% \cmidrule(r){1-1} \cmidrule(rl){2-2}  \cmidrule(rl){3-5}% \cmidrule(rl){6-6} \cmidrule(l){7-8}

$B_F$       & \multirow{7}{*}{USPS}     &  97.8 | 0.17              & 79.4 | 0.97      & 92.3 | 0.60                \\ 
% \cdashline{1-5}
$S_{\text{Distr}}$     &                           &  97.9 | 0.19              & 79.3 | 0.97              & 92.3 | 0.60                \\ 
$S_{\text{Distr}30}$   &                           & 97.9 | 0.18               & \textbf{79.6 | 0.80}     & \textbf{92.7 | 0.51}               \\
$S_{\text{Neigh}}$     &                           & \textbf{98.0 | 0.18}      & 79.4 | 0.97              & 89.4 | 2.12                \\ 
$S_{\text{Neigh}30}$   &                           & 97.9 | 0.20               & 79.3 | 0.83              & 91.2 | 1.21               \\ 
$S_{\text{GAN}}$     &                           & 97.7 | 0.21               & 79.2 | 1.02              & 90.9 | 0.94                \\  
$S_{\text{GAN}30}$   &                           & 97.8 | 0.24               & 79.5 | 0.58              & 91.2 | 0.76                \\  
\bottomrule
\end{tabular}
}

\end{minipage}
\end{table}

% \begin{table}[]
% \begin{minipage}[t]{0.98\textwidth}
% \centering
% {\small
% \begin{tabular}{l|llll|lll}
%                               & \multicolumn{4}{c|}{\textbf{Digit Classification}}                                                                            & \multicolumn{3}{c}{\textbf{Natural Image Classification}}                   \\ \hline
% Population                     & Source                                     & \multicolumn{3}{c|}{Target}                                                      & \multicolumn{1}{l|}{Source}                    & \multicolumn{2}{c}{Target} \\ \hline
% \multicolumn{1}{r|}{\textbf{}} & \multicolumn{1}{r}{\textbf{}}              & \multicolumn{1}{r}{MNIST} & \multicolumn{1}{r}{SVHN} & \multicolumn{1}{r|}{USPS} & \multicolumn{1}{l|}{}                          & CIFAR-10      & STL-10     \\ \hline

% base                           & \multicolumn{1}{l|}{\multirow{7}{*}{SVHN}} & 91.1 | 0.95               & 70.7 | 8.80              & 91.1 | 0.95               & \multicolumn{1}{l|}{\multirow{7}{*}{STL-10}}   &               &            \\
% direct                         & \multicolumn{1}{l|}{}                      & 95.0 | 0.78               & 72.4 | 6.36              & 95.0 | 0.78               & \multicolumn{1}{l|}{}                          &               &            \\
% uniform                        & \multicolumn{1}{l|}{}                      & 91.7 | 1.07               & 70.6 | 4.58              & 91.7 | 1.07               & \multicolumn{1}{l|}{}                          &               &            \\
% train                          & \multicolumn{1}{l|}{}                      & 95.9 | 9.85               & 77.9 | 1.40              & 95.9 | 9.85               & \multicolumn{1}{l|}{}                          &               &            \\
% best                           & \multicolumn{1}{l|}{}                      & 95.5 | 0.68               & 76.4 | 1.02              & 95.5 | 0.68               & \multicolumn{1}{l|}{}                          &               &            \\
% kde\_z\_train                  & \multicolumn{1}{l|}{}                      & 95.0 | 0.81               & 71.8 | 7.68              & 95.0 | 0.81               & \multicolumn{1}{l|}{}                          &               &            \\
% kde\_z\_best                   & \multicolumn{1}{l|}{}                      & 95.5 | 0.40               & 74.2 | 1.39              & 95.5 | 0.40               & \multicolumn{1}{l|}{}                          &               &            \\ \hline
% base                           & \multicolumn{1}{l|}{\multirow{7}{*}{USPS}} & 91.1 | 0.95               & 70.7 | 8.80              & 92.2 | 0.58               &                                                &               &            \\
% direct                         & \multicolumn{1}{l|}{}                      & 97.8 | 0.17               & 97.8 | 0.18              & 92.3 | 0.60               &                                                &               &            \\
% train                          & \multicolumn{1}{l|}{}                      & 98.0 | 0.18               & NaN                      & 89.4 | 2.12               &                                                &               &            \\
% best                           & \multicolumn{1}{l|}{}                      & 97.9 | 0.20               & 79.3 | 0.83              & 91.2 | 1.21               &                                                &               &            \\
% kde\_z\_train                  & \multicolumn{1}{l|}{}                      & 97.9 | 0.19               & NaN                      & 92.3 | 0.60               &                                                &               &            \\
% kde\_z\_best                   & \multicolumn{1}{l|}{}                      & 97.9 | 0.18               & NaN                      & 92.7 | 0.51               &                                                &               &            \\
% uniform                        & \multicolumn{1}{l|}{}                      & NaN                       & NaN                      & 78.8 | 2.23               &                                                &               &           
% \end{tabular}
% \caption{Median accuracy of the populations trained on image classification tasks after fine-tuning. On the main diagonal are in-distribution experiments, otherwise out-of-distribution from source to target. $B_T$ denotes the baseline with 700 members trained directly on the target dataset. The other populations have at least 50 members each. $B_F$ is the second baseline pre-trained on source and fine-tuned on target. $S_{\text{Distr}}$ is the distribution based sampling method, $S_{\text{Neigh}}$ the neighborhood based sampling method. The suffix $30$ indicates that the sampling method was based on the top 30 \% of the train set. Bold numbers highlight the best source-to-target results. Confidence intervals, p-values and effect size can be found in the Appendix.
% \todo{add stderror / CIs | remove second population | remove USPS source}
% }
% \label{tab:gen_hyper_reps:accuracies}
% }
% \end{minipage}
% \end{table}



% \begin{table}[t]
% \begin{minipage}[t]{0.98\textwidth}
% \centering
% {\small
% \begin{tabular}{l|l|ccc|l|l|cc}
% \toprule
% % \multicolumn{5}{c}{\textbf{Version 2 - ID+OOD}}  \\
% \multicolumn{5}{c|}{\texttt{Digit Classification}} & \multicolumn{4}{c}{\texttt{Natural Image Classificationw}}  \\

% \midrule
% Population & Source & \multicolumn{3}{c|}{\texttt{Target}}  & Population & Source & \multicolumn{2}{c}{\texttt{Target}} \\
% \midrule
%             &                           & MNIST             & SVHN              & USPS              &               &                           & CIFAR-10                 & STL-10 \\
% \midrule
% $B_T$       &                           & 0.911              & 0.723            & \textbf{0.922}    & $B_T$         &                           &        0.490             &         0.390 \\
% \midrule
% % $B_T$     & MNIST                     & 0.911               & 0.222           & 0.333 \\ 
% $B_F$       & \multirow{5}{*}{MNIST}    & 0.912               & 0.762           & 0.791             & $B_F$         & \multirow{5}{*}{CIFAR-10} &        0.486             & \textbf{0.428} \\  
% \hdashline
% $S_{\text{Distr}}$     &                           & 0.923               & 0.767           & 0.794             & $S_{\text{Distr}}$       &                           &        0.483             &         0.407 \\
% $S_{\text{Distr}30}$   &                           & 0.931               & \textbf{0.772 } & \textbf{0.808}   & $S_{\text{Distr}30}$     &                           & \textbf{0.487 }          &         0.413  \\
% $S_{\text{Neigh}}$     &                           & 0.934               & 0.768           & 0.789	            & $S_{\text{Neigh}}$       &                           &        0.456             &         0.367  \\
% $S_{\text{Neigh}30}$   &                           & \textbf{0.940}      & 0.770           & 0.796	            & $S_{\text{Neigh}30}$     &                           &        0.462             &         0.379  \\
% \midrule
% $B_F$       & \multirow{5}{*}{SVHN}     & 0.951               & 0.732           & 0.872             &  $B_F$       & \multirow{5}{*}{STL-10}    & \textbf{0.493}  & \textbf{0.395}   \\  
% \hdashline
% $S_{\text{Distr}}$     &                           & 0.951               & 0.730           & 0.872             &  $S_{\text{Distr}}$     &                            & 0.486                     & 0.373   \\ 
% $S_{\text{Distr}30}$   &                           & 0.955               & 0.742           & 0.883             &  $S_{\text{Distr}30}$   &                           & 0.488                      & 0.383   \\ 
% $S_{\text{Neigh}}$     &                           & \textbf{0.972 }     & \textbf{0.781 } & \textbf{0.887 }   &  $S_{\text{Neigh}}$     &                           & 0.100                      & 0.283  \\  
% $S_{\text{Neigh}30}$   &                           & 0.955               & 0.765           & 0.858             &  $S_{\text{Neigh}30}$   &                           & 0.490                      & 0.378   \\  
% \midrule
% $B_F$       & \multirow{5}{*}{USPS}     & 0.978               & 0.795  	          & 0.923 \\ 
% \cdashline{1-5}
% $S_{\text{Distr}}$     &                           &                     & 0.795           & 0.922	 \\ 
% $S_{\text{Distr}30}$   &                           & \textbf{0.980}      & \textbf{0.796 } & \textbf{0.927 }\\
% $S_{\text{Neigh}}$     &                           &                     & 0.795           & 0.900 \\ 
% $S_{\text{Neigh}30}$   &                           & \textbf{0.980}      & 0.792           & 0.913 \\ 
% \bottomrule
% \end{tabular}
% }
% \caption{Median accuracy of the populations trained on image classification tasks after fine-tuning. On the main diagonal are in-distribution experiments, otherwise out-of-distribution from source to target. $B_T$ denotes the baseline with 700 members trained directly on the target dataset. The other populations have at least 50 members each. $B_F$ is the second baseline pre-trained on source and fine-tuned on target. $S_{\text{Distr}}$ is the distribution based sampling method, $S_{\text{Neigh}}$ the neighborhood based sampling method. The suffix $30$ indicates that the sampling method was based on the top 30 \% of the train set. Bold numbers highlight the best source-to-target results. Confidence intervals, p-values and effect size can be found in the Appendix.
% \todo{add stderror / CIs | remove second population | remove USPS source}
% }
% \label{tab:gen_hyper_reps:accuracies}
% \end{minipage}
% \end{table}


% \begin{table}[t]
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% {\small
% \begin{tabular}{l|l|ccc}
% \toprule
% % \multicolumn{5}{c}{\textbf{Version 2 - ID+OOD}}  \\
% \multicolumn{5}{c}{\texttt{Digit Classification - Accuracies}}  \\
% \midrule
% & Source & \multicolumn{3}{c}{\texttt{Target}}  \\
% \midrule
%             &       & MNIST             & SVHN              & USPS \\
% \midrule
% $B_T$       &       & 0.911              & 0.723            & 0.922 \\ 
% \midrule
% % $B_T$     & MNIST & 0.911               & 0.222           & 0.333 \\ 
% $B_F$       & MNIST & 0.912               & 0.763           & 0.796 \\ 
% $S_{\text{Distr}}$     & MNIST & 0.927               & 0.795           & 0.936 \\
% $S_{\text{Distr}30}$   & MNIST & 0.932               & 0.794           & \textbf{0.937 }\\
% $S_{\text{Neigh}}$     & MNIST & 0.932               & \textbf{0.797 } & 0.925	 \\ 
% $S_{\text{Neigh}30}$   & MNIST & \textbf{0.940}      & \textbf{0.794 } & 0.928	 \\ 
% %\midrule
% \midrule
% % $B_T$     & SVHN  & 0.111               & 0.723           & 0.333 \\ 
% %\midrule
% $B_F$       & SVHN  & 0.951               & 0.732           & 0.872  \\ 
% $S_{\text{Distr}}$     & SVHN  & 0.951               & 0.730           & 0.872 \\
% $S_{\text{Distr}30}$   & SVHN  & \textbf{0.955 }     & 0.742           & \textbf{0.883 }\\
% $S_{\text{Neigh}}$     & SVHN  & \textbf{0.972 }     & \textbf{0.781 } & \textbf{0.887 } \\ 
% $S_{\text{Neigh}30}$   & SVHN  & 0.955               &\textbf{0.765 }  & 0.858\\ 
% %\midrule
% \midrule
% % $B_T$     & USPS  & 0.111               & 0.222           & 0.922 \\ 
% %\midrule
% $B_F$       & USPS  & 0.978               & 0.795  	          & 0.922 \\ 
% $S_{\text{Distr}}$     & USPS  & 0.980               & 0.795           & 0.922	 \\ 
% $S_{\text{Distr}30}$   & USPS  & 0.980               & \textbf{0.796 } & \textbf{0.925 }\\
% $S_{\text{Neigh}}$     & USPS  & 0.980               & 0.795           & 0.897 \\ 
% $S_{\text{Neigh}30}$   & USPS  & \textbf{0.980 }     & 0.792           & 0.911 \\ 
% %\midrule
% \midrule
% \end{tabular}
% }
% % \caption{Accuracy of sampled models: median and 95\% confidence intervals. On the main diagonal are in-distribution experiments, otherwise out-of-distribution from source to target. Bold numbers highlight the best source-to-target results. A * denotes cases, in which the boot-strapped CI on the median could not be computed. We report the 95\% CI on the mean instead.}
% % \label{tab:gen_hyper_reps:accuracy_digits}
% \end{minipage}
% % \end{table}
% \hspace{2mm}
% % \begin{table}[t]
% \begin{minipage}[t]{0.48\textwidth}
% \centering
% {\small
% \begin{tabular}{l|l|cc}
% \toprule
% \multicolumn{4}{c}{\texttt{Natural Image Classification - Accuracies}}  \\
% \midrule
% & Source & \multicolumn{2}{c}{\texttt{Target}}  \\
% \midrule
%             & & CIFAR-10 & STL-10 \\
% \midrule
% $B_T$       &  &        0.490             &         0.390 \\
% \midrule
% $B_F$       & CIFAR-10  &        0.486             & \textbf{0.428} \\ 
% $S_{\text{Distr}}$     & CIFAR-10  &        0.483             &         0.407 \\
% $S_{\text{Distr}30}$   & CIFAR-10  & \textbf{0.487 }          &         0.413  \\
% $S_{\text{Neigh}}$     & CIFAR-10  &        0.456             &         0.367  \\
% $S_{\text{Neigh}30}$   & CIFAR-10  &        0.111             &         0.379  \\
% %\midrule
% \midrule
% % $B_T$       & STL-10    & 0.111 [0.111, 0.111] & 0.222 [0.222, 0.222] \\ 
% %\midrule
% $B_F$       & STL-10    & 0.111  & 0.222   \\ 
% $S_{\text{Distr}}$     & STL-10    & 0.111  & 0.222   \\ 
% $S_{\text{Distr}30}$   & STL-10    & 0.111  & 0.222   \\ 
% $S_{\text{Neigh}}$     & STL-10    & 0.111  & 0.222  \\ 
% $S_{\text{Neigh}30}$   & STL-10    & 0.111  & 0.222   \\ 
% \midrule
% \end{tabular}
% }
% % \caption{Accuracy of sampled models: median and 95\% confidence intervals. }
% % \label{tab:gen_hyper_reps:accuracy_natural_images}
% \end{minipage}
% \caption{Accuracy of sampled models: median and 95\% confidence intervals. On the main diagonal are in-distribution experiments, otherwise out-of-distribution from source to target. Bold numbers highlight the best source-to-target results. A * denotes cases, in which the boot-strapped CI on the median could not be computed. We report the 95\% CI on the mean instead.}
% \label{tab:gen_hyper_reps:accuracy_digits}

% \vspace{-.2in}
% \end{table}











% \begin{table}[t]
% \begin{minipage}[t]{0.98\textwidth}
% \centering
% {\small
% \begin{tabular}{l|l|ccc}
% \toprule
% \multicolumn{5}{c}{\textbf{Version 2 - ID+OOD}}  \\
% \multicolumn{5}{c}{\texttt{Digit Classification - Accuracies}}  \\
% \midrule
% & Source & \multicolumn{3}{c}{\texttt{Target}}  \\
% \midrule
%             &       & MNIST                             & SVHN                          & USPS \\
% \midrule
% $B_T$       &       & 0.911 [0.911, 0.912]              & 0.723 [0.720, 0.724]          & 0.922 [0.921, 0.922]\\ 
% \midrule
% % $B_T$     & MNIST & 0.911 [0.911, 0.912]              & 0.222 [0.222, 0.222]          & 0.333 [0.333, 0.333]\\ 
% $B_F$       & MNIST & 0.912 [0.910, 0.913]              & 0.763 [0.758, 0.765]          & 0.796 [0.793, 0.799]*\\ 
% $S_{\text{Distr}}$     & MNIST & 0.927 [0.925, 0.928]              & 0.795 [0.792, 0.797]          & 0.936 [0.935, 0.936]\\
% $S_{\text{Distr}30}$   & MNIST & 0.932 [0.931, 0.933]              & 0.794 [0.792, 0.795]          & \textbf{0.937	[0.936, 0.937]}\\
% $S_{\text{Neigh}}$     & MNIST & 0.932 [0.931, 0.933]              & \textbf{0.797 [0.796, 0.799]} & 0.925	[0.924, 0.927]\\ 
% $S_{\text{Neigh}30}$   & MNIST & \textbf{0.940 [0.939, 0.941]}     & \textbf{0.794 [0.793, 0.796]} & 0.928	[0.926, 0.928]\\ 
% %\midrule
% \midrule
% % $B_T$     & SVHN  & 0.111 [0.111, 0.111]              & 0.723 [0.720, 0.724]          & 0.333 [0.333, 0.333]\\ 
% %\midrule
% $B_F$       & SVHN  & 0.951 [0.950, 0.953]              & 0.732 [0.728, 0.734]          & 0.872 [0.870, 0.874]\\ 
% $S_{\text{Distr}}$     & SVHN  & 0.951 [0.948, 0.951]              & 0.730	[0.726, 0.733]          & 0.872	[0.867, 0.879]\\
% $S_{\text{Distr}30}$   & SVHN  & \textbf{0.955 [0.953, 0.957]}     & 0.742 [0.739, 0.745]          & \textbf{0.883 [0.880, 0.885]}\\
% $S_{\text{Neigh}}$     & SVHN  & \textbf{0.972 [0.970, 0.973]}     & \textbf{0.781 [0.779, 0.782]} & \textbf{0.887 [0.882, 0.889]} \\ 
% $S_{\text{Neigh}30}$   & SVHN  & 0.955 [0.954, 0.957]              &\textbf{0.765 [0.763, 0.767]}  & 0.858 [0.855, 0.861]\\ 
% %\midrule
% \midrule
% % $B_T$     & USPS  & 0.111 [0.111, 0.111]              & 0.222 [0.222, 0.222]          & 0.922 [0.921, 0.922]\\ 
% %\midrule
% $B_F$       & USPS  & 0.978 [0.978, 0.979]              & 0.795 [0.793, 0.797] 	          & 0.922 [0.921*, 0.923*]\\ 
% $S_{\text{Distr}}$     & USPS  & 0.980	[0.979, 0.980]              & 0.795	[0.792, 0.796]          & 0.922	[0.921, 0.923]\\ 
% $S_{\text{Distr}30}$   & USPS  & 0.980 [0.979, 0.980]              & \textbf{0.796 [0.794, 0.797]} & \textbf{0.925 [0.924, 0.926]}\\
% $S_{\text{Neigh}}$     & USPS  & 0.980 [0.979, 0.980]              & 0.795 [0.793, 0.796]          & 0.897 [0.333, 0.333]\\ 
% $S_{\text{Neigh}30}$   & USPS  & \textbf{0.980 [0.980, 0.981]}     & 0.792	[0.790, 0.796]          & 0.911 [0.911, 0.913]\\ 
% %\midrule
% \midrule
% \end{tabular}
% }
% \caption{Accuracy of sampled models: median and 95\% confidence intervals. On the main diagonal are in-distribution experiments, otherwise out-of-distribution from source to target. Bold numbers highlight the best source-to-target results. A * denotes cases, in which the boot-strapped CI on the median could not be computed. We report the 95\% CI on the mean instead.}
% \label{tab:gen_hyper_reps:accuracy_digits}
% \end{minipage}
% \vspace{-.2in}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \begin{minipage}[t]{0.98\textwidth}
% \centering
% {\small
% \begin{tabular}{l|l|cc}
% \toprule
% \multicolumn{4}{c}{\texttt{Natural Image Classification - Accuracies}}  \\
% \midrule
% & Source & \multicolumn{2}{c}{\texttt{Target}}  \\
% \midrule
%             & & CIFAR-10 & STL-10 \\
% \midrule
% $B_T$       &           &        0.490 [0.489, 0.490]            &         0.390 [0.389, 0.391] \\ 
% \midrule
% $B_F$       & CIFAR-10  &        0.486 [0.489, 0.487]            & \textbf{0.428 [0.425, 0.429]} \\ 
% $S_{\text{Distr}}$     & CIFAR-10  &        0.483 [0.481, 0.484]            &         0.407 [0.403, 0.409] 	 \\ 
% $S_{\text{Distr}30}$   & CIFAR-10  & \textbf{0.487 [0.484, 0.488]}          &         0.413 [0.409, 0.415] \\ 
% $S_{\text{Neigh}}$     & CIFAR-10  &        0.456 [0.449, 0.460]            &         0.367 [0.358, 0.374] \\ 
% $S_{\text{Neigh}30}$   & CIFAR-10  &        0.111 [0.111, 0.111]            &         0.379 [0.373, 0.382] \\ 
% %\midrule
% \midrule
% % $B_T$       & STL-10    & 0.111 [0.111, 0.111] & 0.222 [0.222, 0.222] \\ 
% %\midrule
% $B_F$       & STL-10    & 0.111 [0.111, 0.111] & 0.222 [0.222, 0.222] \\ 
% $S_{\text{Distr}}$     & STL-10    & 0.111 [0.111, 0.111] & 0.222 [0.222, 0.222] \\ 
% $S_{\text{Distr}30}$   & STL-10    & 0.111 [0.111, 0.111] & 0.222 [0.222, 0.222] \\ 
% $S_{\text{Neigh}}$     & STL-10    & 0.111 [0.111, 0.111] & 0.222 [0.222, 0.222] \\ 
% $S_{\text{Neigh}30}$   & STL-10    & 0.111 [0.111, 0.111] & 0.222 [0.222, 0.222] \\ 
% \midrule
% \end{tabular}
% }
% \caption{Accuracy of sampled models: median and 95\% confidence intervals. }
% \label{tab:gen_hyper_reps:accuracy_natural_images}
% \end{minipage}
% \vspace{-.2in}
% \end{table}

==> chapters/chapter_5_scalable_hyper_representations/sections/graveyard.tex <==
\paragraph{Tokenization}
In the work by \citet{schurholtSelfSupervisedRepresentationLearning2021}, models are conceptualized as sequences of components, and they propose a method to encode model weights into tokens. Initially, they flatten the weights of each layer along the outgoing dimension, resulting in one weight vector per outgoing channel, which we refer to as "raw tokens." Since the raw tokens from different layers may have varying parameter counts, they employ individual tokenization heads to embed the kernels of these different layers.

In contrast, our approach suggests the use of a fixed token size. If the raw tokens exceed this token size, we split them into several pieces; conversely, if they are smaller, we zero-pad them. This decouples the tokenization process from the representation learning phase, allowing us to embed any model as long as it aligns with the specified token size, without the requirement for learned tokenizers.

To prevent a reconstruction loss due to zero-padding, we incorporate signal masking into the reconstruction loss calculation. Additionally, we propose per-token position encodings consisting of three components: i) the global position of the token within the entire model sequence; ii) the index of the layer; and iii) the index of the token within its respective layer.

\paragraph{Sequences and Windows: Decoupling Memory and Model Size}
The introduction of uniformly-sized tokens in our approach provides a solution to address both memory and compute limitations. This is achieved by conducting learning not on the entire sequence but rather on parts of the sequence, which we refer to as "windows," following conventional sequence learning practices.
\michael{Ditto, what is subsedtions.}\konstantin{replaced with 'part' here, too. Hope that works.}

Utilizing windows on the full model sequence effectively decouples memory requirements from the model's size. The choice of the window size strikes a balance between GPU memory utilization and the necessary contextual information.

To completely separate embeddings from the window size and enable flexibility in using different window sizes during training and inference, we adopt per-token embeddings instead of the global embeddings proposed by \citet{schurholtSelfSupervisedRepresentationLearning2021}. In this approach, after a pass through the encoder transformer, each token ($T_i$) undergoes linear compression to obtain its latent representation 
$L_i=f_C(T_i)$, where $f_c$ represents the linear compression function. 
During decoding, the token is linearly mapped back to the original token size and passed through the decoder transformer as $T_i=f_D(L_i)$, where $f_D$ is the linear decompression.

For the contrastive loss, which guides the training process, we employ a straightforward MLP projection head ($P_{\text{head}}$) with a fixed window size. It maps a window of tokens to embedding $L_{c,j} = P_{\text{head}}(L_{j,\cdots,j+W})$, where $W$ is the fixed window size. The contrastive loss is computed using embeddings $L_{c,j}$ of different views.
\michael{This entire discussion should be a bit more formal, with a few equations at appropriate places.}\konstantin{TODO: add equations forward pass and loss on windows}

It is important to note that this setup allows for the embedding of sequences from various models, which could be further enhanced with additional type or connectivity encodings. However, since our current work focuses on model populations using the same ResNet architecture, we reserve the exploration of such additional encodings for future research endeavors.

To prevent potential overfitting to specific window positions, we propose a strategy of randomly selecting windows from each model sequence multiple times. This approach ensures sufficient coverage of the full sequence for effective representation learning.

\paragraph{Inference on model sequences}
During inference, the reduced memory load permits the utilization of larger windows, potentially extending up to the entire model sequence. However, our investigations reveal that deviating from the training window size leads to a decrease in reconstruction performance. This decline appears to stem from interference between tokens that are too distant from each other and do not co-occur within the same window during training. Consequently, we choose to employ windows during inference as well.

To ensure the generation of coherent and complete samples, we align the borders of these inference windows. Drawing inspiration from the approach outlined in \citet{vaswaniScalingLocalSelfAttention2021}, we introduce a concept known as a "context halo" of tokens. This context halo extends beyond the window boundaries and serves to enhance the consistency between adjacent windows. Importantly, it should be noted that the context tokens are added solely for inference purposes and are disregarded for any other use of the models.

Specifically, the first window is flush with the beginning of the model sequence and has double context at the end. Similarly, the last window is flush with the end of the model sequence and the previous window. The context is used to fill the sequence to the same size as the others, ensuring a uniform treatment of all windows. All windows in between have flush content windows and overlapping context around them.


 

\paragraph{Normalization}
Previous research has emphasized the importance of weight normalization for effective representation learning, as demonstrated in works such as \citet{schurholtHyperRepresentationsGenerativeModels2022} and \citet{peeblesLearningLearnGenerative2022}. However, implementing the loss-normalization scheme described in \citet{schurholtHyperRepresentationsGenerativeModels2022} can become intricate when dealing with windows positioned at variable locations. To address this challenge, we opt for a simpler approach by standardizing the weights per layer across the model population, akin to the per-channel normalization values commonly used in computer vision tasks. 
$\hat{W}_i = \frac{W_i-\mu_i}{\sigma_i}$, where $\mu_i$ and $\sigma_i$ are the per-layer mean and standard deviation across all models in the population.
These standardization values are recorded during \ourmethod training and subsequently employed to de-normalize the weights for generative tasks.

\paragraph{Batch Norm Conditioning}
With the methods outlined above, hyper-representations can be effectively trained to achieve low and evenly distributed reconstruction errors across all layer types. However, we encountered a challenge related to the running statistics of batch-normalization (batch norm) layers. Learning these statistics proved to be challenging and caused issues for both reconstructed and generated models. We hypothesize that this discrepancy arises because batch norm statistics are updated during the forward pass based on the input data, rather than being updated via gradients during training.
\michael{What does ``We hypothesize'' mean?  Are we just saying that?  Or can we test that hypothesis?}\konstantin{Sorry about that, at this point we're just saying that. The intuition is that the reconstruction error on the weights is fairly evenly distributed over layers and layer types. The only real stand out are the running statistics, where the error is large and I couldn't make the model learn.}

We conducted experiments with various normalization schemes for these parameters, but these attempts did not yield satisfactory results. As a solution, we adopted a post-processing step. Assuming access to some data, we perform forward passes with this data through the reconstructed or generated model to update only the batch norm statistics. Importantly, this process does not update the learned weights of the model. It serves to align the batch norm statistics with the model's weights, thereby facilitating the evaluation of its performance.

\paragraph{Bootstrapped Model Sampling}
Previous research has employed the distribution of models with specific targeted properties as anchors for the purpose of sampling. For instance, in \citep{schurholtHyperRepresentationsGenerativeModels2022}, models with high accuracy were used as anchors. However, this approach has two inherent drawbacks: i) it relies on the availability of models possessing the desired properties; ii) the information from such models is confined to the original training domain.

To alleviate these constraints, we propose an alternative method. The methods proposed above significantly enhance the zero-shot performance of sampled models. Consequently, even generated models (before fine-tuning) offer sufficient signal to compare different candidates effectively. Moreover, evaluating a sampled model is relatively cost-effective.
As a result, we introduce a method called \emph{subsampled}. In this approach, we use any suitable model as an initial anchor, sample models broadly, evaluate these sampled models using a target metric, and retain only the best-performing models based on that metric.

Furthermore, this sampling method can be bootstrapped. It involves re-using the embeddings of models that match the desired properties most closely as new anchors. This iterative process updates the distribution from which model embeddings are sampled. We refer to this method as \emph{bootstrapped}.
To eliminate the requirement for anchor models entirely, one can define a prior distribution and sample initial anchor embeddings from that distribution. However, it's essential to note that this approach, while functional to some extent, tends to significantly decrease performance.
\konstantin{consider removing bootstrapped, adding formula to make things clearer.}
